0-1 Integer Linear Programming with a Linear Number of Constraints

We give an exact algorithm for the 0-1 Integer Linear Programming problem with a linear number of constraints that improves over exhaustive search by an exponential factor. Specifically, our algorithm runs in time $2^{(1-\text{poly}(1/c))n}$ where n is the number of variables and cn is the number of constraints. The key idea for the algorithm is a reduction to the Vector Domination problem and a new algorithm for that subproblem.

==> TeX/style/macros.tex <==
\usepackage{amsmath,amsthm,amscd,amsfonts,amssymb,amstexalg}
\usepackage{verbatim}
\usepackage[classfont=bold,langfont=roman,funcfont=italic,basic]{complexity}
\usepackage[dvips]{graphicx}
\usepackage{caption}
\usepackage{color}
\usepackage[colorlinks]{hyperref}

\setlength{\evensidemargin}{-0.0in}
\setlength{\oddsidemargin}{-0.0in}
\setlength{\textwidth}{6.5in}
\setlength{\topmargin}{+0.0in}
\setlength{\textheight}{8.50in}

\theoremstyle{plain}
\newtheorem{thm}{Theorem}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{conjecture}[thm]{Conjecture}
\newtheorem{corollary}[thm]{Corollary}
\newtheorem{proposition}[thm]{Proposition}
\newtheorem{claim}[thm]{Claim}
\newtheorem{fact}[thm]{Fact}
\newtheorem{axiom}{Axiom}

\theoremstyle{definition}
\newtheorem{definition}{\textbf{Definition:}}
\newtheorem{example}{\textbf{Example:}}
\newtheorem{problem}{Problem}

\theoremstyle{remark}
\newtheorem*{remark}{Remark}
\newtheorem*{note}{RNote}
\newtheorem*{notation}{Notation}
\newtheorem*{case}{Case}
\newtheorem*{acknowledgment}{Acknowledgment}
\newtheorem*{summary}{Summary}
\newtheorem*{conclusion}{Conclusion}

%\numberwithin{equation}


\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\ran}{ran}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\Frac}{Frac}
\DeclareMathOperator{\msb}{msb}
\DeclareMathOperator{\lsb}{lsb}

\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\secref}[1]{\S\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}

\newcommand{\prob}{\mathbf{Pr}}
\newcommand{\var}{\mathbf{Var}}
\newcommand{\im}{\mathbf{Image}}

\newcommand{\subexp}{\mathrm{Subexp}}
\newcommand{\exptime}{\mathbf{E}}
\newcommand{\ppoly}{\mathbf{P/poly}}
\newcommand{\expt}{\mathbf{E}}
\newcommand{\sat}{\mathrm{SAT}}
\newcommand{\OR}{\mathrm{OR}}
\newcommand{\AND}{\mathrm{AND}}
\newcommand{\ptime}{\mathbf{P}}
\newcommand{\dtime}{\mathbf{DTIME}}
\newcommand{\ntime}{\mathbf{NTIME}}
\newcommand{\nql}{\mathbf{NQL}}
\newcommand{\ql}{\mathbf{QL}}
\newcommand{\rtime}{\mathbf{RTIME}}
\newcommand{\np}{\mathbf{NP}}
\newcommand{\opp}{\mathbf{OPP}}
\newcommand{\op}{\mathbf{OP}}
\newcommand{\snp}{\mathbf{SNP}}
\newcommand{\conp}{\mathbf{co}\text{-}\mathbf{NP}}
\newcommand{\rp}{\mathbf{RP}}
\newcommand{\rtimeComp}{\mathbf{RTime}}

\newcommand{\prepmach}{\mathbf{PrepMachine}}
\newcommand{\rpsearch}{\mathbf{RPSearch}}
\newcommand{\size}{\mathbf{size}}
\newcommand{\desc}{\mathbf{desc}}
\newcommand{\cktsat}{\mathbf{CircuitSat}}
\newcommand{\turingsat}{\mathbf{TuringSat}}
\newcommand{\speedup}{\mathbf{SpeedUp}}
\newcommand{\nullspace}{\mathbf{Null}}
\newcommand{\rank}{\mathbf{rank}}
\newcommand{\linear}{\mathbf{\tilde{O}(m)}}
\newcommand{\ind}{\rm Independent Set}
\newcommand{\ssl}{\rm Satisfiability Speedup Lemma}
\newcommand{\subExp}{\mathbf{2^{o(n)}}}
\newcommand{\expo}{\mathbf{2^{\alpha n}}}
\newcommand{\ETH}{\mathbf{ETH}}
\newcommand{\SETH}{\mathbf{SETH}}
\newcommand{\bpoly}{\mathbf{m^k}}
%\newcommand{\poly}{\mathrm{poly}}
\newcommand{\prepckt}{\mathbf{PrepCkt}}
\newcommand{\serf}{\mathrm{SERF}}
\newcommand{\sol}{\mathbf{Sol}}

\newcommand{\reals}{\mathbb{R}}
\newcommand{\nnreals}{\mathbb{R}^{\geq 0}}
\newcommand{\ints}{\mathbb{Z}}
\newcommand{\nnints}{\mathbb{Z}^{\geq 0}}
\newcommand{\nats}{\mathbb{N}}
\newcommand{\rats}{\mathbb{Q}}
\newcommand{\dlog}{dlog}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}


\newcommand{\D}{\mathcal{D}}
\newcommand{\Hash}{\mathcal{H}}
%\newcommand{\C}{\mathcal{C}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\B}{\mathcal{B}}


\newcommand{\str}{\structure}


==> TeX/style/packages.tex <==
\usepackage{amsmath,amsthm,amscd,amsfonts,amssymb,amstexalg}
\usepackage{verbatim}
\usepackage[classfont=bold,langfont=caps,funcfont=typewriter,full]{complexity}
\usepackage[dvips]{graphicx}
\usepackage{caption}
\usepackage{color}
\usepackage[colorlinks]{hyperref}




==> TeX/style/size.tex <==
\setlength{\evensidemargin}{-0.0in}
\setlength{\oddsidemargin}{-0.0in}
\setlength{\textwidth}{6.5in}
\setlength{\topmargin}{+0.0in}
\setlength{\textheight}{9.00in}

